Fast Benchmarking of Asynchronous Multi-Fidelity Optimization on Zero-Cost Benchmarks

While deep learning has celebrated many successes, its results often hinge on the meticulous selection of hyperparameters (HPs). However, the time-consuming nature of deep learning training makes HP optimization (HPO) a costly endeavor, slowing down the development of efficient HPO tools. While zero-cost benchmarks, which provide performance and runtime without actual training, offer a solution for non-parallel setups, they fall short in parallel setups as each worker must communicate its queried runtime to return its evaluation in the exact order. This work addresses this challenge by introducing a user-friendly Python package that facilitates efficient parallel HPO with zero-cost benchmarks. Our approach calculates the exact return order based on the information stored in file system, eliminating the need for long waiting times and enabling much faster HPO evaluations. We first verify the correctness of our approach through extensive testing and the experiments with 6 popular HPO libraries show its applicability to diverse libraries and its ability to achieve over 1000x speedup compared to a traditional approach. Our package can be installed via pip install mfhpo-simulator.

==> appendices/wrapper-args.tex <==
\section{Wrapper Object (\texttt{ObjectiveFuncWrapper})}
\label{appx:wrapper:section}
In this section, we describe more details on our wrapper.

\subsection{Arguments}
\label{appx:wrapper-args:section}
The arguments of \texttt{ObjectiveFuncWrapper} object are as follows:
\begin{itemize}
  \vspace{-1.5mm}
  \item \texttt{obj\_func}: the objective function that takes (\texttt{eval\_config}, \texttt{fidels}, \texttt{seed}, \texttt{**data\_to\_scatter}) as arguments and returns $f(\xv|\av)$ and $\tau(\xv|\av)$ where \texttt{eval\_config} is \texttt{dict[str, Any]},
  \vspace{-1.5mm}
  \item \texttt{launch\_multiple\_wrappers\_from\_user\_side (bool)}: whether to instantiate multiple wrappers from userside (e.g. NePS that uses file-based synchronization) or not (e.g. DEHB that uses multiprocessing that spawns subprocesses),
  \vspace{-1.5mm}
  \item \texttt{ask\_and\_tell (bool)}:
  whether to use simulator for ask-and-tell interface (\texttt{True}) or not,
  \vspace{-1.5mm}
  \item \texttt{save\_dir\_name (str | None)}: the results and the required information will be stored in \texttt{mfhpo-simulator-info/<save\_dir\_name>/},
  \vspace{-1.5mm}
  \item \texttt{n\_workers (int)}: the number of parallel workers $P$,
  \vspace{-1.5mm}
  \item \texttt{n\_evals (int)}: the number of evaluations to get,
  \vspace{-1.5mm}
  \item \texttt{n\_actual\_evals\_in\_opt (int)}: the number of HP configurations to be evaluated in an optimizer which is used only for checking if no hang happens (should take \texttt{n\_evals + n\_workers}),
  \vspace{-1.5mm}
  \item \texttt{continual\_max\_fidel (int | None)}:  when users would like to restart each evaluation from intermediate states, the maximum fidelity value for the target fidelity must be provided.
  Note that the restart is allowed only if there is only one fidelity parameter.
  If \texttt{None}, no restart happens as in Line~\ref{main:methods:line:continual-eval} of Algorithm~\ref{main:methods:alg:automatic-job-alloc-wrapper},
  \vspace{-1.5mm}
  \item \texttt{runtime\_key (str)}: the key of the runtime in the returned value of \texttt{obj\_func},
  \vspace{-1.5mm}
  \item \texttt{obj\_keys (list[str])}: the keys of the objective and constraint names in the returned value of \texttt{obj\_func} and the values of the specified keys will be stored in the result file,
  \vspace{-1.5mm}
  \item \texttt{fidel\_keys (list[str] | None)}: the keys of the fidelity parameters in input \texttt{fidels},
  \vspace{-1.5mm}
  \item \texttt{seed (int | None)}: the random seed to be used in the wrapper,
  \vspace{-1.5mm}
  \item \texttt{max\_waiting\_time (float)}: the maximum waiting time for each worker and if each worker did not get any update for this amount of time, it will return \texttt{inf},
  \vspace{-1.5mm}
  \item \texttt{store\_config (bool)}: whether to store configurations, fidelities, and seed used for each evaluation, and
  \vspace{-1.5mm}
  \item \texttt{check\_interval\_time (float)}: how often each worker should check whether a new job can be assigned to it.
  \vspace{-1.5mm}
\end{itemize}
Note that \texttt{data\_to\_scatter} is especially important when an optimizer uses multiprocessing packages such as \texttt{dask} or \texttt{multiprocessing}, which deserialize \texttt{obj\_func} every time we call.
By passing large-size data via \texttt{data\_to\_scatter}, the time for (de)serialization will be negligible if optimizers use \texttt{dask.scatter} or something similar internally.
We kindly ask readers to check any updates to the arguments at
\ifunderreview
\url{https://anonymous.4open.science/r/mfhpo-simulator-3C81/README.md}.
\else
\url{https://github.com/nabenabe0928/mfhpo-simulator/}.
\fi

\subsection{Wrapper for Ask-and-Tell Interface}
\label{appx:wrapper-ask-and-tell:section}
When optimizers take ask-and-tell interface, simulations can be run on a single worker while preserving the results, and hence simulations can be further accelerated.
Note that the bottleneck of simulations is the waiting time due to the communication among each worker and simulations on a single worker can address this problem.
The benefits of this option are (1) faster, (2) memory-efficient, and (3) stable.
On the other hand, the downsides are that (1) this option forces optimizers to have the ask-and-tell interface and (2) simulations may fail to precisely consider a bottleneck caused by parallel execution of expensive optimizers.
For more details, see \url{https://github.com/nabenabe0928/mfhpo-simulator/}.


==> sections/validation/edge-case.tex <==
\subsection{Visual Verification on Small Handcrafted Test Cases}
\label{main:validation:section:small-cases}

In this section, we will check our wrapper on the following small handcrafted cases:
\begin{enumerate}
  \item the cheap optimizer with $\{\taun{n}\} = \{100,40,30,20,20,30,40,20,20,30,20,40,30,20,$\linebreak $30,20,30,40,30,10\}$,
  \item the expensive optimizer with $\{\taun{n}\} = \{40,60,60,50,50,30,30,30\}$, and
  \item the expensive optimizer with $\{\taun{n}\} = \{50,130,80,160,130,70,20,30\}$.
\end{enumerate}
Note that the expensive optimizer uses $c = 10$.
\figref{main:validation:fig:cumtime-match-on-toy} shows that the results obtained using our wrapper do not contradict to our intuition, e.g., each worker starts evaluation one after another and each worker waits for another samplings for the other workers.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.98\textwidth]{figs/cumtime-match.pdf}
  \caption{
    The results of the experiments on small handcrafted cases obtained by our wrapper.
    The $x$-axis shows the simulated runtime of each experiment and the $y$-axis has four horizontal lines, which represent the timelines for each worker.
    We can see that our wrapper gives the expected timelines for each worker.
    \textbf{Left}: the test case with the cheap optimizer.
    \textbf{Center}: the test case with the expensive optimizer and a sequence of HP configurations that causes waiting before some samplings.
    As expected, each sampling waits for the end of the previous sampling.
    \textbf{Right}: the test case with the expensive optimizer and a sequence of HP configurations that does not cause any waiting.
    As expected, each sampling starts immediately after each evaluation.
  }
  \label{main:validation:fig:cumtime-match-on-toy}
\end{figure}

==> settings/labels-in-main.tex <==
\ifappendix
% Do nothing

\else

% Define the labels in the main sections
\customlabel{data1}{1}
\customlabel{data2}{2}

% Start numberings of each data as if
% appendix takes over the numbering from the main section
\renewcommand\thefigure{\arabic{figure}}
\setcounter{figure}{1}  % start from 2
\renewcommand\thetable{\arabic{table}}
\setcounter{table}{2}  % start from 3
\renewcommand\thealgorithm{\arabic{algorithm}}
\setcounter{algorithm}{3}  % start from 4
\renewcommand\theequation{\arabic{equation}}
\setcounter{equation}{4}  % start from 5

% Change the numbering of sections to Alphabetic
\renewcommand{\thesection}{\Alph{section}} 
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesection.\arabic{subsection}.\arabic{subsubsection}}

\fi

